PRICE: A Pretrained Model for Cross-Database Cardinality Estimation

Cardinality estimation (CardEst) is essential for optimizing query execution plans. Recent ML-based CardEst methods achieve high accuracy but face deployment challenges due to high preparation costs and lack of transferability across databases. In this paper, we propose PRICE, a PRetrained multI-table CardEst model, which addresses these limitations. PRICE takes low-level but transferable features w.r.t. data distributions and query information and elegantly applies self-attention models to learn meta-knowledge to compute cardinality in any database. It is generally applicable to any unseen new database to attain high estimation accuracy, while its preparation cost is as little as the basic one-dimensional histogram-based CardEst methods. Moreover, PRICE can be finetuned to further enhance its performance on any specific database. We pretrained PRICE using 30 diverse datasets, completing the process in about 5 hours with a resulting model size of only about 40MB. Evaluations show that PRICE consistently outperforms existing methods, achieving the highest estimation accuracy on several unseen databases and generating faster execution plans with lower overhead. After finetuning with a small volume of databasespecific queries, PRICE could even find plans very close to the optimal ones. Meanwhile, PRICE is generally applicable to different settings such as data updates, data scaling, and query workload shifts. We have made all of our data and codes publicly available at https://github.com/StCarmen/PRICE.

==> plots/table_of_baselines.tex <==
% \begin{smaller}
\begin{scriptsize}
\begin{table}[htbp]
\centering
% \begin{threeparttable}
\caption{Properties of different methods}

% \vspace{-11pt}
\setlength\tabcolsep{2.5pt}

\resizebox{\columnwidth}{!}{%
\arrayrulecolor{black}
\begin{tabular}{c|c|c|c|c|c|c|c}

\hline

{Method} & \tabincell{c}{Data-\\driven} &  \tabincell{c}{Query-\\driven} & \tabincell{c}{Space\\Overhead} & \tabincell{c}{Inference\\Time} & \tabincell{c}{Read for Un-\\seen Datasets} & \tabincell{c}{Prepare for Un-\\seen Datasets} & \tabincell{c}{Preparation \\Time}  \\ \hline


PG~\cite{postgresql} & $\checkmark$ & $\times$ & {low} & {low} & $\checkmark$ & {Statistics} & {low} \\ \hline

DeepDB~\cite{DBLP:journals/pvldb/HilprechtSKMKB20} & $\checkmark$ & $\times$ & {high} & {medium} & $\times$ & {Modeling} & {medium} \\ \hline

NeuroCard~\cite{DBLP:journals/pvldb/YangKLLDCS20} & $\checkmark$ & $\times$ & {high} & {high} & $\times$ & {Modeling} & {medium} \\ \hline

FactorJoin~\cite{DBLP:journals/pacmmod/WuNAKM23} & $\checkmark$ & $\times$ & {small} & {high} & $\times$ & {Modeling} & {medium} \\ \hline

MSCN~\cite{DBLP:conf/cidr/KipfKRLBK19} & $\checkmark$ & $\checkmark$ & {small} & {low} & $\times$ & {Statistics + Workload + Training} & {high} \\ \hline

ALECE~\cite{li_alece_2023} & $\checkmark$ & $\checkmark$ & {high} & {small} & $\times$ & {Statistics + Workload + Training} & {high} \\ \hline

OURS & $\checkmark$ & $\checkmark$ & {medium} & {small} & $\checkmark$ & {Statistics + Finetuning (option)} & {small} \\ \hline
\end{tabular}
} % resizebox
\begin{flushleft}
\begin{tablenotes}[para]\footnotesize
% \item Note: Preparation for Un-seen Datasets involves: 
\item Statistics: Accumulates essential statistical data from the database.\\
\item Workload: Collects training workloads from database transactions.\\
\item Training: Uses deep learning to create predictive models from training data.\\
\item Modeling: Builds models reflecting distribution and relations. Queries independent.
\end{tablenotes}
\end{flushleft}
% \end{threeparttable}
% \vspace{-3pt}
\end{table}
% \end{smaller}
\end{scriptsize}


==> sections/model.tex <==

\begin{figure*} 
\includegraphics[width=\linewidth]{figures/model.pdf}
\vspace{-20pt}
\captionsetup{font=large}
\caption{\ModelName Structure}
\label{fig:model}
\end{figure*} 

\section{\ModelName}
\label{sec:model}

\note{We outline the structure and components of our proposed Pretrained Multi-Table CardEst Model (\ModelName) in Figure~\ref{fig:model}. On a high level, \ModelName applies a number of features in low-dimensional space w.r.t.~each attribute and widely adapts to any database. Then, the model learns to simulate the CardEst process and condense such meta-knowledge as learned parameters. We briefly explain the features applied in \ModelName and its workflow as follows and we further explore the cross-database applicability of \ModelName.}

\subsection{Feature Selection}
\label{sec:model-feature}
For a database $D$ and a SQL query $Q$, our model takes four classes of features  as follows.

1) \emph{The value distribution of each attribute $\Pr(A_{i, j})$, i.e.~a vector of histogram, occurring in join conditions or predicates in $Q$.} 
Such histogram vectors are regarded as basic \emph{tokens} in our approach. They resemble the word embeddings in the NLP models as they could be combined with learned parameters to recover the high-level joint PDF $\Pr(T_{Q})$~\cite{li_alece_2023}. 
\note{For categorical attributes, we utilize the SpaceSaving Summary\cite{10.1145/1166074.1166084} to maintain the distribution, which guarantees error-bound estimates and supports real-time updates. }
To eliminate the different ranges of attributes, we normalize each histogram vector or summary vector to span into $[0, 1]$. 
We also encode the size $|T_i|$ of each table to characterize its volume.


2) \emph{The distribution of the scaling factors of each join condition $T_i.A_{i, x} = T_j.A_{j, y}$ in $Q$.}
Let $s$ be a tuple in table $T_i$. The \emph{scaling factor} of $s$ refers to how many of tuples $t$ in table $T_j$ could join with $s$, i.e.~$s[A_{i, x}] = t[A_{j, y}]$. Such distributions are also encoded as histogram vectors. As they capture the inter-table correlation information, they could help the model to learn how to scale $\Pr(T_i)$ to $\Pr(T_{Q})$ (see details in Eq.~(1) in~\cite{DBLP:journals/pvldb/ZhuWHZPQZC21}). 

3) \emph{The information of each filtering predicate}
 ``$T_i.A_{i, j} \textsc{ op value} $'' \emph{in Q}. 
We encode: i) the range of the filtering \textsc{value} by its lower and upper bound. 
\note{For categorical attributes, the index of the bin corresponding to the value is utilized as the range. In cases of equivalent queries, where the predicate is an equality, both the lower and upper bounds are set to the same value. To standardize across different attribute scales, we normalize the filtering range to span from $[0, 1]$.
and ii) the selectivity, calculated as the ratio of tuples satisfying the predicate on attribute $A_{i, j}$ over all tuples in $T_i$. This aids in computing $\Pr(Q)$ from the joint PDF.
Additional heuristic estimators(see details in ~\cite{DBLP:journals/pvldb/DuttWNKNC19}), such as AVI, EBO, and MinSel, provide simplified single-table selectivity estimates. . }

4) \emph{The query-level information of $Q$}, including:
i) the number of joins and filters in $Q$;
ii) the structural properties of $Q$ by considering its join graph, such as its diameter and maximum degree;
and iii) the cardinality estimated by traditional methods, e.g.~the histogram-based methods in PostgreSQL.
These would provide more guidelines to distinguish different queries and produce better results.

Notably, all the above features could be easily obtained in a total cost $O(\sum_{i} |T_i|)$. Thus, our \ModelName is as cheap as the efficient traditional histogram-based methods in terms of feature construction. 


\subsection{Workflow of \ModelName}
\label{sec:model-model}

In the initial step, \ModelName combines the information w.r.t.~each attribute $A_{i, j}$ using simple linear models. Specifically, if $A_{i, j}$ occurs in the join condition, it combines its value distribution and the scaling factor distribution vector together as an embedding vector $L_{i, j}$; if $A_{i, j}$ occurs in the predicates of query $Q$, the linear model combines its value distribution, filtering range and selectivity to output the embedding vector $P_{i, j}$. 
\note{Notably, linear parameters are shared among features of the same type.
Additionally, we initialize a "query token" -- akin to the CLS token in Natural Language Processing (NLP) or a virtual node in Graph Neural Networks (GNN). This token serves to amalgamate the comprehensive representation of $\Pr(Q)$ throughout the learning process, functioning as a pivotal component in synthesizing query-level insights.
The query token is randomly initialized and subsequently transformed into an embedding vector, denoted as $R$, within the embedding layer. The dimensions for $L$, $P$, and $R$ are uniformly fixed, ensuring uniformity across different types of embeddings.}

Then, \ModelName apply two main stages to exploit the capabilities of attention mechanisms to obtain key information for CardEst computation. 


\note{In the \emph{scaling stage}, the query token $R$ and embedding vectors $L_{i, j}$ -- representing each attribute $A_{i, j}$ in the join condition—are fed into the model. 
\ModelName applies self -- attention model to convert $R$ and each $L_{i, j}$ into new embedding vectors, $R'$ and $L'{i, j}$, respectively.  
Each $L'_{i, j}$ is a weighted sum over $L_{i, j}$ and all other vectors $L_{i', j'}$. The weight for each pair of input vector $L_{i', j'}$ to the output vector $L'_{i, j}$, a.k.a.~attention coefficients, are determined by learned parameters. Similarly, The new query token, $R'$, is derived as a weighted sum of all $L_{i, j}$ vectors. 
This architecture allows the model to adeptly handle queries featuring various numbers of join attributes by dynamically adjusting the focus of the attention mechanism based on the query structure.
Using such attentions, the output vectors $R'$ capture the correlations between the scaling factor distributions of different joins in $Q$, which reflect 
how the scaling factors are combined when multiple tables are joined together. Upon such knowledge, the model could know how to scale the low-level joint PDF $\Pr(T_{i})$ on each single table to the high-level joint PDF $\Pr(T_{Q})$ on the joined table. Moreover, each $L'_{i, j}$ is engineered to consider the impact of other attribute distributions during the join process, thereby refining the approximation of $\Pr(A'_{i,j})$ within $\Pr(T_{Q})$.  This can provide attribute $A_{i,j}$ a better representation for the next stage when interacting with the filter condition.}

\note{In the \emph{filtering stage}, the focus shifts to  obtaining the information of $\Pr(T_{Q})$ and computing the probability $\Pr(Q)$. Recall that each embedding vector $P_{i, j}$ condenses the value distribution and filtering information on attribute $A_{i, j}$. Let $U =  \{P_{i, j}\} \cup \{ L'_{i', j'} \}$ be the set of all embedding vectors $P_{i, j}$ and $L'_{i, j}$. We apply an attention mechanism between the query token $R'$ and all vectors in $U$. In similar, for each pair of vectors $u, v \in U$, we compute an attention coefficient as weight using the same learned parameters. Then for each $u \in U$, we obtain the embedding vector $u'$ using weighted sum over all vectors in $U$. This operation not only fuses the scaling information from multiple tables as encoded in $L'{i, j}$ but also integrates the value distributions of all attributes in $Q$ as encoded in $P{i, j}$. This comprehensive amalgamation effectively captures the details of $\Pr(T_{Q})$.
Furthermore, the vectors $u'$ integrate the filtering predicate information with $\Pr(T_{Q})$, providing a new representation after filtered.
The refined query token representation, $R''$, emerging from this stage encapsulates all relevant information about join conditions and filter conditions, thereby offering a renewed and enriched representation of the query. 
Consequently, \ModelName is equipped to compute $\Pr(Q)$ from $\Pr(T_{Q})$, leveraging the integrated and detailed attribute interactions and filtering effects.}

\note{In the final step, we feed vectors $R''$ and all auxiliary query-level features into a multilayer perceptron (MLP)~\cite{DBLP:books/lib/HastieTF09}  to obtain the desired cardinality estimation $\hat{\Card}(Q)$.}




\subsection{Cross-Database Applicability of \ModelName}
\label{sec:model-analysis}

\note{
This subsection delves into the aspects of \ModelName that enable its effective use across different database environments, highlighting its adaptability and robustness in handling diverse datasets.}

\note{
\stitle{Transferable Featurization.}
\ModelName utilizes a set of features (as detailed in Section ~\ref{sec:model-feature}) that are universally available and maintain consistent meanings across various databases. By normalizing these features, we effectively resolve discrepancies in magnitude between databases, mapping disparate database features into a unified feature space. This standardization is crucial for the model to assimilate generalizable knowledge, thereby enhancing its predictive accuracy across different database.}


\note{
\stitle{Adaptive Attention Mechanism.}
Attention mechanisms~\cite{DBLP:conf/nips/VaswaniSPUJGKP17} fundamentally transform model processing by selectively concentrating on relevant aspects of input data while disregarding the irrelevant, thereby mimicking human cognitive attention processes. Essentially, these mechanisms compute attention weights that act as significance scores for different parts of the input data. These weights are crucial in determining the emphasis placed on various input segments during the formation of representations or predictions. The application of these weights produces a weighted sum, or context vector, which distills crucial information into a format that the model can efficiently use. This dynamic focus enables models to adapt to the intricacies and relevance of specific data points, enhancing both the accuracy and depth of data interpretation.}

\note{
In practical terms, attention mechanisms significantly enhance the model's adaptability and efficiency, particularly in scenarios requiring the handling of inputs with variable lengths—such as different numbers of joins and filters in database queries. Unlike traditional neural network architectures that necessitate fixed-size inputs, attention mechanisms inherently accommodate varying input sizes without the need for padding or truncation, maintaining data integrity and computational efficiency. Moreover, by providing a mechanism to examine the relevance scores, attention also boosts the interpretability of the model, offering insights into which data features the model finds most informative. Additionally, we do not use positional encoding~\cite{DBLP:conf/nips/VaswaniSPUJGKP17}, in contrast to the attention structure commonly used in the NLP domain, as there is no sequentiality between all join conditions and all filter conditions in the query.}

\note{
\stitle{Handling Data Updates and Workload Drift.}
Data updates and workload drift pose significant challenges to the stability of cardinality estimation models. 
To address data updates, our approach involves a straightforward update of the statistical features utilized by the model. These features, such as histograms and summaries, are designed to support real-time updates. This capability allows for the maintenance of each attribute's features with minimal storage requirements and the rapid integration of these updated features during the query-to-vector transformation process, ensuring efficiency and reducing time consumption.}

\note{
Workload drift can typically manifest in two forms: 1) encountering filters on previously unseen attributes or new filter constants, and 2) an increase in the number of join or filter conditions. For the first scenario, our model does not rely on traditional one-hot encoding, which hardcodes attribute values. Instead, it characterizes each attribute by its distribution, allowing the model to effectively handle new or unseen attribute if it has encountered similar distributions during pre-training. For the second scenario, our experimental findings confirm that the model's performance remains stable regardless of the quantity of join and filter conditions involved in query(detailed in Section~\ref{sec:exp-robust}). This stability is attributed to the attention mechanism's capability to dynamically adjust to variable-length inputs and selectively focus on the most relevant data features, thus enhancing the model's adaptability and robustness in varying databases.}




In summary, \ModelName is a very general method. On one side, by applying the attention mechanism, it could process queries with any number of joins, tables and predicates on attributes with any distribution. On the other side, \ModelName learns the key information to simulate the CardEst computation process from the statistical perspective. As long as it is well trained to on a variety of databases, the model parameters could capture the meta-knowledge to do CardEst in different settings. 
Thus, we could seamlessly apply \ModelName on any dynamic and unseen new database with low cost of preparations. 
Further, \ModelName also reserves the flexibility to fit for each specific database through fine-tuning. In this way, its performance could be further improved. As verified by our evaluation results in Section~\ref{sec:exp-finetune}, 
the original \ModelName could already achieve commendable performance on unseen databases, while the fine-tuned \ModelName could attain state-of-the-art performance.

% \subsection{Challenge of Query Representation}
% \label{sec:featurization-challenge}

% 必须清楚地阐明传统方法的不足之处，尤其是在处理现代数据库环境的复杂性和数据不断变化的性质方面。包括传统方法失效的具体实例或场景尤其具有启发性。

% 如今CardEst model采用的query representation方法虽然看上去各有特色，但大多都基于传统的one-hot编码方式，

% query representation：可以在介绍自己的query表征前详细说明一下旧的方法为什么不适配
% 1. one-hot编码决定了需要预先知道有多少个列，从而生成对应长的向量表示，这样的话如果database新增了列就没办法handle了，而unseen database一定会出现训练集中未见过的列。
% 2. one-hot编码没办法直接标识到未见过的列，即使给未见过的列新增一个标识，但model在训练过程中并没有学习过和该标识相关的任何信息，所以也不可能对其作出准确的估计
% 3. one-hot编码的query表征如果不加入db相关的信息，那么模型只能隐式地去学习这些列与列之间的相关性，一旦列的分布发生了变动，one-hot编码并不会产生改变，但对应的列与列之间的相关性却发生了改变直接导致最终cardinality发生了变动，现有的机器学习模型大多都只能对相同的x预测出一个结果，但其对应的label却发生了改变，估计自然就不准确了。
% 3.传统的workload-driven的方法大多只纳入了sql表征的信息，没有纳入底层数据的信息，底层数据之间的关系全靠模型隐式地去学习，在单一的database上这个方法有效，但因为我们要面对任意unseen的database，这要求我们需要将底层的db信息和关联关系显式地提供给模型，帮助模型学习的同时，能够提高模型在unseen database上的泛化能力。

% 这可能是确立您的方法的价值和创新性的最关键部分。它不仅要断言，还要通过逻辑和证据证明，为什么您的查询表示方法在未见过的数据集上是稳健的。这可能包括讨论所用特征的通用性、模型对新数据分布的适应性，以及与其他方法的潜在比较，以突出您的方法的优势。
